APOLLO: SGD-like Memory, AdamW-level Performance

Large language models (LLMs) are notoriously memory-intensive during training, particularly with the popular AdamW optimizer. This memory burden necessitates using more or higher-end GPUs or reducing batch sizes, limiting training scalability and throughput. To address this, various memory-efficient optimizers have been proposed to reduce optimizer memory usage. However, they face critical challenges: (i) reliance on costly SVD operations; (ii) significant performance trade-offs compared to AdamW; and (iii) still substantial optimizer memory overhead to maintain competitive performance. In this work, we identify that AdamW's learning rate adaptation rule can be effectively coarsened as a structured learning rate update. Based on this insight, we propose Approximated Gradient Scaling for Memory-Efficient LLM Optimization (APOLLO), which approximates learning rate scaling using an auxiliary low-rank optimizer state based on pure random projection. This structured learning rate update rule makes APOLLO highly tolerant to further memory reductions while delivering comparable pre-training performance. Even its rank-1 variant, APOLLO-Mini, achieves superior pre-training performance compared to AdamW with SGD-level memory costs. Extensive experiments demonstrate that the APOLLO series performs on-par with or better than AdamW, while achieving greater memory savings by nearly eliminating the optimization states of AdamW. These savings provide significant system-level benefits: (1) Enhanced Throughput: 3x throughput on an 8xA100-80GB setup compared to AdamW by supporting 4x larger batch sizes. (2) Improved Model Scalability: Pre-training LLaMA-13B with naive DDP on A100-80GB GPUs without system-level optimizations. (3) Low-End GPU Friendly Pre-training: Pre-training LLaMA-7B on a single GPU using less than 12 GB of memory with weight quantization.

==> algs/galore.tex <==



% Define custom colors
\definecolor{highlightcolor}{rgb}{1.0, 0.8, 0.8}  % light red

\begin{algorithm}[tb]
   \caption{Adam with Galore}
   \label{alg:low_rank_adam}
 \begin{algorithmic}
   \STATE {\bfseries Input:} A layer weight matrix $W \in \mathbb{R}^{m \times n}$ with $m \leq n$. Step size $\eta$, scale factor $\alpha$, decay rates $\beta_1, \beta_2$, rank $r$, subspace change frequency $T$.
   \STATE Initialize first-order moment $M_0 \in \mathbb{R}^{n \times r} \gets 0$
   \STATE Initialize second-order moment $V_0 \in \mathbb{R}^{n \times r} \gets 0$
   \STATE Initialize step $t \gets 0$

    % Define a function for SVD and projector initialization
   \STATE {\bf Function} InitializeProjector($G_t$, $r$)
   \STATE \hspace{1.5em} \colorbox{highlightcolor}{$U, S, V \gets \text{SVD}(G_t)$}\COMMENT{\ding{202}}
   \STATE \hspace{1.5em} \colorbox{highlightcolor}{$P_t \gets U[:, :r]$} \COMMENT{Initialize left projector as $m \leq n$}
   \STATE {\bf End Function}
   
   \REPEAT
   \STATE $G_t \in \mathbb{R}^{m \times n} \gets - \nabla_W \phi_t(W_t)$ 
   \IF{$t \bmod T = 0$}
   \STATE {\bf InitializeProjector}($G_t$, $r$)
   \ELSE
   \STATE $P_t \gets P_{t-1}$ \hfill \COMMENT{Reuse the previous projector}
   \ENDIF
   \STATE $R_t \gets P_{t}^{\top} G_t$ \hfill \COMMENT{Project gradient into compact space}
   \\\hrulefill
   \STATE {\bfseries Update $R_t$ by Adam}
    \STATE \hspace{1.5em}$M_t \gets \beta_1 \cdot M_{t-1} + (1 - \beta_1) \cdot R_t$
    \STATE \hspace{1.5em}$V_t \gets \beta_2 \cdot V_{t-1} + (1 - \beta_2) \cdot R_t^2$
    \STATE \hspace{1.5em}$M_t \gets M_t / (1 - \beta_1^t)$
    \STATE \hspace{1.5em}$V_t \gets V_t / (1 - \beta_2^t)$
    \STATE \hspace{1.5em}$N_t \gets M_t / (\sqrt{V_t} + \epsilon)$
   \\\hrulefill
   \STATE \colorbox{highlightcolor} {$\tilde G_t \gets \alpha \cdot P N_t$} \hfill \COMMENT{Project back to original space}
   \STATE \colorbox{highlightcolor}{$W_t \gets W_{t-1} + \eta \cdot \tilde G_t$}
   \STATE $t \gets t + 1$
   \UNTIL{convergence criteria met}
    \STATE \textbf{return} $W_T$
   

   
 \end{algorithmic}
\end{algorithm}
